[OIII] emission in z=2 quasars with and without Broad Absorption Lines

Understanding the links between different phases of outflows from active galactic nuclei is a key goal in extragalactic astrophysics. Here we compare [OIII] $\lambda\lambda$4960,5008 outflow signatures in quasars with and without Broad Absorption Lines (BALs), aiming to test how the broad absorption troughs seen in the rest-frame ultraviolet are linked to the narrow line region outflows seen in the rest-frame optical. We present new near-infrared spectra from Magellan/FIRE which cover [OIII] in 12 quasars with 2.1 < z < 2.3, selected to have strong outflow signatures in CIV $\lambda$1550. Combining with data from the literature, we build a sample of 73 BAL, 115 miniBAL and 125 non-BAL QSOs with 1.5 < z < 2.6. The strength and velocity width of [OIII] correlate strongly with the CIV emission properties, but no significant difference is seen in the [OIII] emission-line properties between the BALs, non-BALs and miniBALs once the dependence on CIV emission is taken into account. A weak correlation is observed between the velocities of CIV BALs and [OIII] emission, which is accounted for by the fact that both outflow signatures correlate with the underlying CIV emission properties. Our results add to the growing evidence that BALs and non-BALs are drawn from the same parent population and are consistent with a scenario wherein BAL troughs are intermittent tracers of persistent quasar outflows, with a part of such outflow becoming optically thick along our line-of-sight for sporadic periods of time within which BALs are observed.

==> O3_tab1.tex <==
J010754.95-095744.2 & BAL & 19.1 & 2587 & 2.146 & 18.55 & 17.37 & -- & 16.14 & VHS & 90\\ 
J011934.27+052629.7 & BAL & 17.5 & 3302 & 2.343 & 18.93 & 17.48 & 16.77 & 15.99 & UKIDSS & 80\\ 
J014725.50-101438.9 & non-BAL & 17.8 & 4128 & 2.153 & 17.09 & 16.12 & 15.36 & 14.78 & 2MASS & 30\\ 
J022943.90-003458.0 & BAL & 26.3 & 2903 & 2.147 & 18.19 & 17.01 & 16.51 & 15.68 & VHS & 60\\ 
J025345.28-080353.3 & BAL & 24.7 & 3874 & 2.109 & 18.41 & 17.26 & -- & 15.96 & VHS & 90\\ 
J094748.06+193920.0 & non-BAL & 16.3 & 5613 & 2.279 & 17.78 & 16.98 & 16.46 & 15.78 & 2MASS & 60\\ 
J100711.80+053208.8 & BAL & 26.1 & 1622 & 2.145 & 16.18 & 15.16 & 14.62 & 13.85 & UKIDSS & 20\\ 
J103546.02+110546.4 & non-BAL & 32.1 & 1115 & 2.365 & 17.26 & 15.77 & 15.10 & 14.23 & UKIDSS & 20\\ 
J120508.10+013455.8 & BAL & 29.7 & 2155 & 2.161 & 18.21 & 16.64 & 16.06 & 15.30 & VIKING & 40\\ 
J120550.19+020131.5 & BAL & 17.3 & 5108 & 2.156 & 16.94 & 16.02 & 15.61 & 15.00 & VIKING & 40\\ 
J121328.78-025617.8 & BAL & 24.5 & 5136 & 2.176 & 17.84 & 16.95 & 16.42 & 15.69 & VIKING & 60\\ 
J123647.13+185311.3 & non-BAL & 14.7 & 4859 & 2.128 & 17.64 & 16.69 & -- & 15.32 & 2MASS & 40\\ 

